28 GHz mmWave Channel Measurements and Modeling in a Library Environment

To fully exploit the millimeter-wave bands for the fifth generation cellular systems, an accurate understanding of the channel propagation characteristics is required, and hence extensive measurement campaigns in different environments are needed. In this paper, we use a rotated directional antenna-based channel sounder for measurements at 28 GHz in large indoor environments at a library setting. We present models for power angular-delay profile and large-scale path loss based on the measurements over distances ranging from 10 m to 50 m. In total, nineteen different line-of-sight (LOS) and non-line-of-sight (NLOS) scenarios are considered, including the cases where the transmitter and the receiver are placed on different floors. Results show that the close-in free space reference distance and the floating intercept path loss models both perform well in fitting the empirical data. The path loss exponent obtained for the LOS scenarios is found to be very close to that of the free space path loss model.

==> Fatih_Ozgur_Library Measurements_RWS_2020/head.tex <==
%This is the head.tex file you need.
%\fnsymbol{footnote}

\newcommand{\postscript}[2]{
    \par
    \hbox{
           \vbox to #1{
           \vfil
           \special{#2.ps}
         }
    }
}
\let\ssstyle=\scriptscriptstyle
\newcommand{\define}{\newcommand}
\newcommand{\bt}{\begin{tabular}}
\newcommand{\et}{\end{tabular}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bel}[1]{\be\label{#1}}
\newcommand{\bd}{\begin{displaymath}}
\newcommand{\ed}{\end{displaymath}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bn}{\begin{enumerate}}
\newcommand{\en}{\end{enumerate}}
\newcommand{\bds}{\begin{description}}
\newcommand{\eds}{\end{description}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bqa}{\begin{eqnarray}}
\newcommand{\eqa}{\end{eqnarray}}
\newcommand{\sts}{\stackrel{\sim}}
\define{\ul}{\noindent \underline}
\define{\Gamb}{{\bf \Gamma}}
\define{\Sigb}{{\bf \Sigma}}
\define{\Lambs}{{\bf \Lambda}_{s}}
\define{\LambR}{{\bf \Lambda}_{R}}
\define{\OmB}{{\bf \Omega}_{oB}}
\define{\Omo}{{\bf \Omega}_o}
\define{\Omb}{{\bf \Omega}}
\define{\Oms}{{\bf \Omega}_s}
\define{\alpb}{{\bf \alpha}}
\define{\alpbb}{\bar{\bf \alpha}}
\define{\betb}{{\bf \beta}}
\define{\betbb}{\bar{\bf \beta}}
\define{\tr}{\mbox{Tr}}
\define{\CR}{Cram\'{e}r-Rao~}
\define{\Mu}{{\it MUSIC}}
\define{\ES}{{\it ESPRIT}}
\define{\Mi}{{\it Min-Norm}}
\define{\SR}{{\it Subspace Rotation}}
\define{\ath}{{{\bf a}(\theta_k)}}
\define{\Ath}{{\bf A}(\theta)}
\define{\AthH}{{\bf A}^{H}(\theta)}
\define{\athd}{{{\bf a}^{(1)}(\theta_k)}}
\define{\bo}{{\bf 1}}
\define{\bz}{{\bf 0}}
\define{\ab}{{\bf a}}
\define{\bb}{{\bf b}}
\define{\cb}{{\bf c}}
\define{\cbb}{\bar{\bf c}}
\define{\db}{{\bf d}}
\define{\eb}{{\bf e}}
\define{\ebb}{\bar{\bf e}}
\define{\ebk}{{\bf e}_k}
\define{\ebbk}{\bar{\bf e}_k}
\define{\fb}{{\bf f}}
\define{\gb}{{\bf g}}
\define{\hb}{{\bf h}}
\define{\mb}{{\bf m}}
\define{\nb}{{\bf n}}
\define{\ob}{{\bf o}}
\define{\pb}{{\bf p}}
\define{\qb}{{\bf q}}
\define{\rb}{{\bf r}}
\define{\sbb}{{\bf s}}
\define{\tb}{{\bf t}}
\define{\ub}{{\bf u}}
\define{\vb}{{\bf v}}
\define{\wb}{{\bf w}}
\define{\st}{{\bf s}}
\define{\xb}{{\bf x}}
\define{\yb}{{\bf y}}
\define{\zb}{{\bf z}}
\define{\Ab}{{\bf A}}
\define{\Psib}{{\bf \Psi}}
\define{\Xib}{{\bf \Xi}}
\define\sN{{\ssstyle N}}
\define\sM{{\ssstyle M}}
\define\sF{{\ssstyle F}}
\define\sT{{\ssstyle T}}
\define\sH{{\ssstyle H}}
\define\sK{{\ssstyle K}}
\define\sL{{\ssstyle L}}
\define\sP{{\ssstyle P}}
\define\sQ{{\ssstyle Q}}
\define\sV{{\ssstyle V}}
\define{\Au}{{\Ab^{\uparrow}}}
%\define{\Ad}{{\Ab^{\downarrow}}}
\define{\Af}{{\bf A}_F}
\define{\As}{{\bf A}_S}
\define{\Bb}{{\bf B}}
%\define{\Bbb}{{\bar{\bf B}}}
\define{\Cb}{{\bf C}}
\define{\Cbh}{\hat{\bf C}}
\define{\Db}{{\bf D}}
\define{\Eb}{{\bf E}}
%\define{\Es}{{\bf E}_{s}}
\define{\Fb}{{\bf F}}
\define{\Gb}{{\bf G}}
\define{\Hb}{{\bf H}}
\define{\Ib}{{\bf I}}
% \define{\If}{{\bf I}_F}
\define{\Is}{{\bf I}_S}
\define{\Ibd}{{\bf I}^{\downarrow}}
\define{\Ibu}{{\bf I}^{\uparrow}}
\define{\Jb}{{\bf J}}
\define{\Kb}{{\bf K}}
\define{\Lb}{{\bf L}}
\define{\Lbb}{\bar{\bf L}}
\define{\Mb}{{\bf M}}
\define{\Nb}{{\bf N}}
\define{\Ob}{{\bf O}}
\define{\Pb}{{\bf P}}
\define{\Qb}{{\bf Q}}
\define{\Rb}{{\bf R}}
\define{\Rbh}{\hat{\bf R}}
%\define{\Rsh}{\hat{\bf R}_s}
\define{\Rsd}{\Delta {\bf R}_s}
\define{\Rba}{{\bf R}_A}
%\define{\Rbe}{{\bf R}}
\define{\Rbse}{\stackrel{\sim}{{\bf R}_{s}}}
\define{\Rbb}{\bar{\bf R}}
\define{\Sb}{{\bf S}}
\define{\Tb}{{\bf T}}
\define{\Ub}{{\bf U}}
\define{\Vb}{{\bf V}}
\define{\Vn}{{\bf V_n}}
\define{\Wb}{{\bf W}}
\define{\Xb}{{\bf X}}
\define{\Yb}{{\bf Y}}
\define{\Zb}{{\bf Z}}
\define{\thb}{{\bf \Theta}}
\define{\Yd}{\Delta {\bf Y}}
\define{\Yt}{\tilde{\bf Y}}
\define{\Ut}{\tilde{\bf U}}
\define{\Vt}{\tilde{\bf V}}
\define{\Unt}{\tilde{\bf U}_o}
\define{\unt}{\tilde{\bf u}_o}
\define{\Ust}{\tilde{\bf U}_s}
\define{\ust}{\tilde{\bf u}_s}
\define{\Wt}{\tilde{\bf W}}
\define{\Wd}{\Delta \bf {W}}
\define{\Phb}{{\bf {\Phi}}}
\define{\Omegab}{{\bf {\Omega}}}
\define{\Gammab}{{\bf {\Gamma}}}
\define{\Phib}{{\bf {\Phi}}}
\define{\Phd}{\Delta \bf {\Phi}}
\define{\Phl}{{{\bf \Phi}^{\downarrow}}}
\define{\Phu}{{{\bf \Phi}^{\uparrow}}}
%\define{\Psb}{\bf {\Psi}}
\define{\Psd}{\Delta \bf {\Psi}}
\define{\rt}{\tilde{r}}
\define{\rd}{\Delta r}
\define{\td}{\Delta \theta}
\define{\tl}{\tilde{\theta}}
\define{\ut}{\tilde{\bf u}}
\define{\Und}{\Delta {\bf U}_o}
\define{\Usd}{\Delta {\bf U}_s}
\define{\Us}{{\bf U}_s}
\define{\us}{{\bf u}_s}
\define{\Uo}{{\bf U}_o}
\define{\uo}{{\bf u}_o}
\define{\Vs}{{\bf V}_s}
\define{\vs}{{\bf v}_s}
\define{\Vo}{{\bf V}_o}
\define{\vo}{{\bf v}_o}
\define{\Aa}{||{\bf \alpha}_k||^{2}}
\define{\Usx}{{\bf U}_{sx}}
\define{\Usy}{{\bf U}_{sy}}
\define{\Usxd}{\Delta {\bf U}_{sx}}
\define{\Usyd}{\Delta {\bf U}_{sy}}
\define{\Usxt}{\tilde{\bf U}_{sx}}
\define{\Usyt}{\tilde{\bf U}_{sy}}
\define{\Usz}{{\bf U}_{sz}}
\define{\Uszd}{\Delta {\bf U}_{sz}}
\define{\Uszt}{\tilde{\bf U}_{sz}}
\define{\Ft}{\tilde{\bf F}}
\define{\Fd}{\Delta {\bf F}}
\define{\At}{\tilde{\bf A}}
%\define{\Ade}{\Delta {\bf A}}
\define{\Bt}{\tilde{\bf B}}
\define{\Bd}{\Delta {\bf B}}
\define{\ld}{\Delta \bar{\lambda}_k}
\define{\ldd}{\Delta \lambda_k}
\define{\lt}{\tilde{\lambda}}
\define{\lb}{\bar{\lambda}}
%\define{\ut}{\ul{\triangle}}
\define{\df}{\stackrel{\rm def}{=}}
\define{\diag}{\rm diag}
\define{\prf}{\noindent \underline{Proof:}\\}
\define{\pe}{\hfill $\Box$}
\define{\doi}{\stackrel{j\neq i}{j=1}}
\define{\dok}{\stackrel{j\neq k}{j=1}}
\define{\ds}{\displaystyle}
\define{\Usu}{{\bf U}_s^{\uparrow}}
\define{\Usl}{{\bf U}_s^{\downarrow}}
\define{\Unu}{{\bf U}_o^{\uparrow}}
\define{\Unl}{{\bf U}_o^{\downarrow}}
\define{\Oo}{{\bf \Omega}_{o}}
\define{\Ot}{{\tilde{\bf \Omega}}_{o}}
\define{\Os}{{\bf \Omega}_{s}}
\define{\Ou}{{\bf O}^{\uparrow}}
\define{\Od}{{\bf O}^{\downarrow}}
\define{\thd}{\Delta \theta}
\define{\Iu}{{\bf I}^{\uparrow}}
\define{\Il}{{\bf I}^{\downarrow}}
%\define{\Otu}{ {{\tilde{\bf O}}^{\uparrow}} }
\define{\Otd}{{\tilde{\bf O}}^{\downarrow}}
\define{\Sr}{{\bf \Sigma}_s^{{1}\over{2}}}
\define{\Sp}{{\bf \Sigma}_s^{-1}}
\define{\Ss}{{\bf \Sigma}_s^{-{{1}\over{2}}}}
\define{\nun}{\underline{\bf n}}
\define{\nh}{\bar{\bf n}}
\define{\eq}[1]{(\ref{#1})}
\define{\dB}{\delta {\bf B}}
\define{\deb}{\delta b}
\define{\bul}{\underline{\beta}}
\define{\ape}{\stackrel{\cdot}{=}}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{observation}{Observation}
\newtheorem{property}{Property}
\newtheorem{definition}{Definition}
\newcommand{\vsp}{\rule[-1.5ex]{0ex}{4.1ex}}
\define{\im}{\,\mbox{Im}}
\define{\re}{\,\mbox{Re}}

\define{\rmE}{\mathrm{E}}
\define{\rme}{\mathrm{e}}
\newcommand{\Expect}[1]{\mathop{\mathbb{E}}\left[ #1 \right ]}
%usage: \Expect{x}


==> Fatih_Ozgur_Library Measurements_RWS_2020/latexmkrc.tex <==
$pdflatex = 'pdflatex %O %S; ps2pdf14 -dPDFSETTINGS=/prepress %B.pdf %B-embed.pdf; mv %B-embed.pdf %B.pdf';

==> Fatih_Ozgur_Library Measurements_RWS_2020/myhead.tex <==
\let\ssstyle=\scriptscriptstyle
\def\sN{{\ssstyle N}}
\def\sd{{\ssstyle d}}
\def\s0{{\ssstyle 0}}
\def\sM{{\ssstyle M}}
\def\sF{{\ssstyle F}}
\def\sT{{\ssstyle T}}
\def\sH{{\ssstyle H}}
\def\sK{{\ssstyle K}}
\def\sL{{\ssstyle L}}
\def\sP{{\ssstyle P}}
\def\sQ{{\ssstyle Q}}
\def\sV{{\ssstyle V}}
\def\trg{{\triangle}}
\def\Rcal{{\cal R}}
\def\sgn{{\rm sgn}}
\define{\Pib}{{\bf \Pi}}
% \define{\bs}{\begin{slide}}
% \define{\es}{\end{slide}}
\define{\xz}{\epsilon_{l,0}(n)}
\define{\xx}{\epsilon_{l,1}(n)}
\define{\xc}{\epsilon_{l,2}(n)}
%\define{\bi}{\begin{iteize}}
%\define{\ei}{\end{itemize}}


==> latexmkrc.tex <==
$pdflatex = 'pdflatex %O %S; ps2pdf14 -dPDFSETTINGS=/prepress %B.pdf %B-embed.pdf; mv %B-embed.pdf %B.pdf';
